Reproducible Research in Network Modeling

Background: When we model networks, there is a problem of obtaining experimental data to verify other model approaches. And even if there are some experimental data, it is necessary to be sure of their reliability. Purpose: It is necessary to propose methods for obtaining reliable experimental data. Method: By its nature, network equipment is a software and hardware complex. Therefore, a full-scale software model can be considered completely equivalent to real equipment. And a real experiment can be replaced by a nature experiment. The reliability of a nature experiment will be based on its reproducibility. Results A comparison of popular nature network modeling packages was carried out. These packages were divided by functionality and feasibility of reproducible studies. Conclusions: Most software packages meet the reproducibility criteria. The choice of a specific solution depends on non-technical factors: popularity and knowledge of the package.

==> bib/bibtool/include/doi <==
# Convert URL DOI to DOI
#rewrite.rule = {url# "https?://.*doi"} # Should have DOI field instead
#rewrite.rule = {url# "https?://.*doi\.org/\(10\.[0-9]+/[^\"}]+\)" # "{\1}"}
rename.field {url=doiurl if url="doi"}
rename.field {doiurl=delete if doi="10."}
delete.field = {delete}
rename.field {doiurl=doi}
rewrite.rule = {doi# "https?://.*doi\.org/\(10\.[0-9]+/.+\)"# "\1"}


==> bib/bibtool/include/month <==
#
# This resource file tries to introduce BibTeX strings for month names.
# Provisions are made to preserve other information contained in the
# month field.
#

rewrite.rule { month = "^[\"{] *\(.*\)january\(.*\) *[\"}]$" # "{\1} # 1 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)february\(.*\) *[\"}]$" # "{\1} # 2 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)march\(.*\) *[\"}]$" # "{\1} # 3 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)april\(.*\) *[\"}]$" # "{\1} # 4 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)may\(.*\) *[\"}]$" # "{\1} # 5 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)june\(.*\) *[\"}]$" # "{\1} # 6 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)july\(.*\) *[\"}]$" # "{\1} # 7 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)august\(.*\) *[\"}]$" # "{\1} # 8 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)september\(.*\) *[\"}]$" # "{\1} # 9 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)october\(.*\) *[\"}]$" # "{\1} # 10 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)november\(.*\) *[\"}]$" # "{\1} # 11 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)december\(.*\) *[\"}]$" # "{\1} # 12 # {\2}" }

rewrite.rule { month = "^[\"{] *\(.*\)jan\(.*\) *[\"}]$" # "{\1} # 1 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)feb\(.*\) *[\"}]$" # "{\1} # 2 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)mar\(.*\) *[\"}]$" # "{\1} # 3 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)apr\(.*\) *[\"}]$" # "{\1} # 4 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)may\(.*\) *[\"}]$" # "{\1} # 5 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)jun\(.*\) *[\"}]$" # "{\1} # 6 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)jul\(.*\) *[\"}]$" # "{\1} # 7 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)aug\(.*\) *[\"}]$" # "{\1} # 8 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)sep\(.*\) *[\"}]$" # "{\1} # 9 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)oct\(.*\) *[\"}]$" # "{\1} # 10 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)nov\(.*\) *[\"}]$" # "{\1} # 11 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)dec\(.*\) *[\"}]$" # "{\1} # 12 # {\2}" }

rewrite.rule { month = "^{ *} # " = ""}
rewrite.rule { month = " # { *}$" = ""}


==> image/reproducible-network-research/en/Makefile <==
PLANTUML_FIG := $(wildcard *.pu)
pdf_files := $(patsubst %.pu, %.pdf, $(PLANTUML_FIG))
png_files := $(patsubst %.pu, %.png, $(PLANTUML_FIG))

all: $(pdf_files) $(png_files)

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,thm,rel,*~} *eps-converted-to.pdf *.synctex.gz
	-rm -f split*
	rm -rf out auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done

cleanall: clean
	-rm $(pdf_files)

%.svg : %.pu
	-plantuml -nbthread auto -tsvg $<

%.pdf : %.svg
	-rsvg-convert -d 600 -p 600 -u -f pdf $< -o $@

%.png : %.svg
	-rsvg-convert -d 600 -p 600 -u -f png $< -o $@


==> image/reproducible-network-research/ru/Makefile <==
PLANTUML_FIG := $(wildcard *.pu)
pdf_files := $(patsubst %.pu, %.pdf, $(PLANTUML_FIG))
png_files := $(patsubst %.pu, %.png, $(PLANTUML_FIG))

all: $(pdf_files) $(png_files)

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,thm,rel,*~} *eps-converted-to.pdf *.synctex.gz
	-rm -f split*
	rm -rf out auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done

cleanall: clean
	-rm $(pdf_files)

%.svg : %.pu
	-plantuml -nbthread auto -tsvg $<

%.pdf : %.svg
	-rsvg-convert -d 600 -p 600 -u -f pdf $< -o $@

%.png : %.svg
	-rsvg-convert -d 600 -p 600 -u -f png $< -o $@

